Tip of the Tongue Known-Item Retrieval: A Case Study in Movie Identification

While current information retrieval systems are effective for known-item retrieval where the searcher provides a precise name or identifier for the item being sought, systems tend to be much less effective for cases where the searcher is unable to express a precise name or identifier. We refer to this as tip of the tongue (TOT) known-item retrieval, named after the cognitive state of not being able to retrieve an item from memory. Using movie search as a case study, we explore the characteristics of questions posed by searchers in TOT states in a community question answering website. We analyze how searchers express their information needs during TOT states in the movie domain. Specifically, what information do searchers remember about the item being sought and how do they convey this information? Our results suggest that searchers use a combination of information about: (1) the content of the item sought, (2) the context in which they previously engaged with the item, and (3) previous attempts to find the item using other resources (e.g., search engines). Additionally, searchers convey information by sometimes expressing uncertainty (i.e., hedging), opinions, emotions, and by performing relative (vs. absolute) comparisons with attributes of the item. As a result of our analysis, we believe that searchers in TOT states may require specialized query understanding methods or document representations. Finally, our preliminary retrieval experiments show the impact of each information type presented in information requests on retrieval performance.

==> search_intermediation.tex <==
\section{Search Intermediation}\label{sec:experiment}

This study is based on TOT search requests mined from community question-answering websites where the search is performed with the help of human intermediaries. Next, we study the usefulness of standard IR tools in this intermediary function.
In spite of the growing proportion of natural language questions in commercial search logs~\citep{pang2011search} and the increased academic interest in conversational search scenarios~\citep{anand2020conversational}, typical IR models are still designed and optimized for short keyword-based queries. We expect that the TOT questions meant for human intermediaries are suboptimal for querying standard IR systems. The quality of retrieval also depends on what type of information is available in the collection.
For example, the \plotdata collection contains plot descriptions from movies. Therefore, any information in the TOT questions about the exact context in which the user interacted with the target movie is unlikely to help retrieve the right result from this collection. We analyse standard Okapi BM25~\citep{robertson2009probabilistic} as a search intermediary for TOT search requests to gain and validate such insights.

\subsection{Methods}\label{sec:intermediation:methods}

We index the \plotdata collection using Indri~\citep{strohman2005indri} with stopword removal and krovetz stemming.
We extract the search requests from three datasets: \irememberthismoviedata, \namethatmoviedata, and \redditdata, and generate corresponding queries using three different query formulation strategies:
\begin{enumerate*}[label=(\roman*)]
    \item use request title as query,
    \item use request description as query, and
    \item use a concatenation of request title and description as query.
\end{enumerate*}

We employ Okapi BM25 as the retrieval model.
For each dataset, we use $20\%$ of the queries to tune the $k_1$ and $b$ hyperparameters of the BM25 model and evaluate on the remaining heldout $80\%$ of the queries.
We report mean reciprocal rank (MRR) and Success@10 for each run.

To understand how different information in the TOT search requests influences retrieval performance, we also conduct an ablation study against the \irememberthismoviedata collection, where we obtained sentence level annotations for the requests.
We use the combination of request title and description as our baseline query formulation policy and then selectively drop all sentences with specific annotations at a time to measure the impact of their exclusion on search result quality.

\subsection{Results}\label{sec:intermediation:results}
Table \ref{tab:retrieval-overall} summarizes the retrieval performance across all three datasets.
In all cases, we find that request description is more effective as query compared to the request title, but the combination of the two achieves best retrieval performance. On \namethatmoviedata and \redditdata, the BM25 model is able to retrieve the correct movie in the top ten ranks about a quarter of the time, whereas on \irememberthismoviedata we observe success in the top ten positions in less than one-fifth of the cases. The low success rate may be explained by the fact that these requests were formulated for human intermediaries, not keyword based search systems.

\begin{table}[t]
\caption{Retrieval experiments with different query formulation strategies.
For each dataset and each metric, we perform paired student's t-tests to check for statistical significance between all pairs of query formulation strategies.
We find that all the differences are statistically significant ($p < 0.01$) after Bonferroni correction, except ``Description'' \vs ``Title + Description'' on MRR on the \irememberthismoviedata dataset.}
\label{tab:retrieval-overall}
\centering
%{\footnotesize
\begin{tabular}{lrr}
\toprule
  & MRR & Success@10 \\ 
  \midrule
  \irememberthismoviedata \\
  \tabindent Title & $0.025$ & $0.051$ \\
  \tabindent Description & $0.095$ & $0.147$ \\
  \tabindent Title + description & $0.105$ & $0.183$ \\
  \namethatmoviedata \\
  \tabindent Title & $0.075$ & $0.120$ \\
  \tabindent Description & $0.124$ & $0.190$ \\
  \tabindent Title + description & $0.171$ & $0.254$ \\
  \redditdata\\
  \tabindent Title & $0.061$ & $0.112$ \\
  \tabindent Description & $0.128$ & $0.207$ \\
  \tabindent Title + description & $0.161$ & $0.267$ \\
  \bottomrule
\end{tabular}
%}
\end{table}

To study how different information in search requests impact retrieval when a search system is employed as the intermediary we consider the findings from the ablation study summarized in Table \ref{tab:retrieval-annotation}.
For each annotation type, we report both absolute and relative differences, against the baseline query formulation, within the segment of queries where at least one sentence has that particular annotation.

We find that sentences containing information about the movie are generally useful for retrieval, and their exclusion negatively impacts retrieval quality.
In particular, most questions specify a character ($98.2\%$), object ($82.3\%$), scene ($89.7\%$), and location type ($73.7\%$) and dropping sentences containing these information show large degradation in retrieval performance. In contrast, we find that removing sentences that are about social niceties do not have any meaningful impact on retrieval while removing context information seems to improve retrieval performance.

\begin{table}[]
\caption{Ablation experiments on \irememberthismoviedata.  MRR using title and description queries excluding sentences by the most frequent annotation labels using only those questions containing a sentence with that annotation. \bm{The previous sentence seems a bit complicated to read.} Rows sorted within category by absolute difference with respect to the baseline.  Larger drops in performance indicate important sentence types.}
\label{tab:retrieval-annotation}
    \centering
\begin{tabular}{lccccc}\toprule
&&\multicolumn{2}{c}{sentences}&\multicolumn{2}{c}{difference} \\
	&	frequency	&	all	&	ablated	&	absolute	&	relative	\\
\hline
Movie (all)	&	100.0\%	&	0.0840	&	0.0238	&	-0.060	&	-71.7\%	\\
\tabindent Character	&	98.2\%	&	0.0855	&	0.0208	&	-0.065	&	-75.7\%	\\
\tabindent Object	&	82.3\%	&	0.0918	&	0.0303	&	-0.062	&	-67.0\%	\\
\tabindent Scene	&	89.7\%	&	0.0888	&	0.0363	&	-0.053	&	-59.1\%	\\
\tabindent Location type	&	73.7\%	&	0.1002	&	0.0479	&	-0.052	&	-52.2\%	\\
\tabindent Plot summary	&	61.7\%	&	0.1021	&	0.0745	&	-0.028	&	-27.0\%	\\
\tabindent Genre/tone	&	34.8\%	&	0.0498	&	0.0383	&	-0.011	&	-23.1\%	\\
\tabindent Category	&	92.0\%	&	0.0859	&	0.0760	&	-0.010	&	-11.5\%	\\
\tabindent Release date	&	43.4\%	&	0.0581	&	0.0526	&	-0.005	&	-9.5\%	\\
\tabindent Language	&	23.9\%	&	0.0686	&	0.0714	&	0.003	&	4.1\%\\
\tabindent Visual style	&	34.2\%	&	0.1014	&	0.1044	&	0.003	&	3.0\%\\
\\
Context (all)	&	64.9\%	&	0.0779	&	0.0898	&	0.012	&	15.3\%	\\
\tabindent Temporal context	&	57.8\%	&	0.0847	&	0.0995	&	0.015	&	17.5\%	\\
\tabindent Physical medium	&	35.7\%	&	0.0763	&	0.0912	&	0.015	&	19.5\%	\\
\\
Other \\
\tabindent Uncertainty	&	88.5\%	&	0.0790	&	0.0625	&	-0.017	&	-20.9\%	\\
\tabindent Relative comparison	&	20.6\%	&	0.0340	&	0.0277	&	-0.006	&	-18.5\%	\\
\tabindent Social	&	51.6\%	&	0.0398	&	0.0405	&	0.001	&	1.8\%\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Discussion}

\textbf{What information helps search systems?}
The information contained in search requests can have different impact on retrieval based on:
\begin{enumerate*}[label=(\roman*)]
    \item What information is present in the collection appropriate for matching, and
    \item How well the search system can take advantage of the information specified in the request.
\end{enumerate*}

For example, it is not surprising that removal of context information seems to improve retrieval metrics as the \plotdata collection only contains plot descriptions but none of the movie metadata.
Therefore, the provided context information in the search request is unlikely be useful in discriminating between a relevant and nonrelevant result.
A prerequisite to be able to take advantage of the context information in TOT search requests would be to include structured item metadata in our collection, and potentially employ fielded-matching models~\citep{robertson2004simple, zamani2018neural} for retrieval.

Removing sentences with language annotation also do not degrade MRR.
Based on a close reading of the data, it appears that in most cases the mentioned language is English, which may not be very informative for retrieval because of the high proportion of English movies in the \plotdata collection.
Also, when the word ``English'' occurs in \plotdata, it is generally in the context of a plot or scene description, and not to denote the language of the movie---\eg, ``He then uses his computer skills to translate the book from Latin into English'' and ``Sher Singh admits he isn't fluent in English''.

We find that removing sentences annotated with Uncertainty degrades retrieval performance.
This indicates that even when the searcher may be unsure, the stated movie description may be accurate and useful for retrieval.
For example, for the sentence ``I saw the movie somewhere around 1986-88 on TV about young (high school) musician boy who played electronic music on a keyboard'', we find term matches with the correct movie plot description that also contains the phrase ``electronic music''.
Similarly, sentences that make relative comparisons can also often include important keywords that matches with the target movie plot description. For example, the sentence ``I dont know if this Laika was the original Laika who travelled to the space in the 50s or the name is in honor of the real astronaut dog'' contains the terms ``space'' and ``dog'' that matches with the target movie plot description.
Therefore, the inclusion of this sentence in the query formulation on the whole seems to have a positive effect on retrieval---in spite of also including terms like ``Laika'' that appears in 11 other plot descriptions in our collection different from the target movie and may be considered as a distractor in this situation.

It should be noted that the simple IR model employed in our experiments is neither designed to appropriately handle uncertainty nor relative comparisons in search requests.
Ideally, the expressed uncertainty should influence the importance of matching certain attributes that the user may recollect imperfectly.
Similarly, terms included for relative comparisons should be treated differently than attributes that describe the target movie.
From an algorithm design perspective, these indicate opportunities for specialized query understanding and motivate better design of search systems more suitable for handling TOT requests.
